Benchmarking Foundation and Large Language Models for Few-Shot Medical Image Segmentation

Few-shot medical image segmentation (FS-MIS) aims to segment novel regions of interest (ROIs) from a few annotated support examples. Despite rapid progress, existing FS-MIS solutions span diverse paradigms but are evaluated under inconsistent settings, leaving their relative effectiveness unclear. We introduce FAME, a unified benchmark for evaluating FS-MIS solutions, covering specialists, SAM-based methods, CLIP-based methods, and MLLM-based methods. FAME contains 14,958 test samples across 7 anatomical sites, 9 imaging modalities, and 14 ROI categories, and evaluates models under zero-shot and ten-shot settings with additional assessment of target-absence recognition and generalization under covariate and semantic shifts. Our evaluation reveals several findings. First, effective few-shot segmentation depends on how models exploit support examples: direct visual adaptation generally outperforms prompt-based strategies. Second, increasing support examples improves performance only when models can effectively utilize them. Third, semantic transfer remains substantially more challenging than imaging-domain adaptation, and strong localization ability does not necessarily imply reliable target-absence recognition. We hope FAME provides a comprehensive understanding of current FS-MIS solutions and facilitates the development of more effective and reliable few-shot medical segmentation methods.

==> tables/ExistBenchmark.tex <==
\begin{table}[t]
\centering

\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Benchmark} &
\textbf{Domain} &
\textbf{SEG} &
\textbf{Task Opt.} \\

\midrule
\multicolumn{4}{@{}l}{\textit{General few-shot segmentation}} \\
FSS-1000~\cite{li2020fss1000} \textcolor{gray}{CVPR'20}
& General & \cmark & \xmark \\
CD-FSS~\cite{lei2022crossdomain} \textcolor{gray}{ECCV'22}
& General & \cmark & \xmark \\
PerSeg~\cite{zhang2024persam} \textcolor{gray}{ICLR'24}
& General & \cmark & \cmark \\
LVIS-$92^i$~\cite{liu2024matcher} \textcolor{gray}{ICLR'24}
& General & \cmark & \xmark \\


\midrule
\multicolumn{4}{@{}l}{\textit{Medical few-shot segmentation}} \\
UniMedDB~\cite{zhao2026segmic} \textcolor{gray}{Pattern Recognit.'26}
& Medical & \cmark & \xmark \\
MeCoVQA-S~\cite{shen2026image} \textcolor{gray}{TPAMI'26}
& Medical & \cmark & \xmark \\
\textbf{\benchmark~(ours)}
& \textbf{Medical} & \cmark & \cmark \\

\bottomrule
\end{tabular}
}
\caption{Comparison with existing few-shot benchmarks. \textit{Task Opt.} indicates whether the evaluation explicitly optimizes model parameters using the few-shot annotations from the target task.}
\label{tab:fewshot_benchmark}
\end{table}

==> tables/organ_results_iid.tex <==
\begin{table*}[!htbp]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccccccc}
\toprule
& & \multicolumn{2}{c}{\textbf{Brain}} & \multicolumn{2}{c}{\textbf{Breast}} & \multicolumn{2}{c}{\textbf{Colon}} & \multicolumn{2}{c}{\textbf{Retina}} & \textbf{Lung} & \textbf{Skin} & \textbf{Thyroid} & \textbf{Avg} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
\textbf{Method} & \textbf{Adaptation} & Dice & Rej. & Dice & Rej. & Dice & Rej. & Dice & Rej. & Dice & Dice & Dice & Dice \\
\midrule
\multicolumn{14}{l}{\emph{Zero: training-free, no task-specific trainable parameters}} \\
\midrule
MedSAM3 & Zero & \underline{0.375} & \underline{0.083} & \textbf{0.761} & \underline{0.000} & \textbf{0.816} & \underline{0.000} & 0.155 & 0.008 & \textbf{0.736} & \textbf{0.894} & \textbf{0.782} & \textbf{0.646} \\
MedPLIB & Zero & \textbf{0.400} & 0.000 & \underline{0.417} & \underline{0.000} & 0.340 & \underline{0.000} & 0.135 & 0.000 & \underline{0.158} & \underline{0.825} & 0.332 & \underline{0.372} \\
GLaMM & Zero & 0.129 & 0.000 & 0.351 & \underline{0.000} & 0.369 & \underline{0.000} & \textbf{0.164} & 0.000 & 0.043 & 0.645 & \underline{0.417} & 0.302 \\
STAMP-7B & Zero & 0.068 & \underline{0.083} & 0.338 & \underline{0.000} & \underline{0.388} & \underline{0.000} & 0.148 & 0.000 & 0.059 & 0.654 & 0.359 & 0.287 \\
STAMP-2B & Zero & 0.063 & 0.000 & 0.240 & \underline{0.000} & 0.346 & \underline{0.000} & \underline{0.157} & 0.000 & 0.052 & 0.614 & 0.287 & 0.251 \\
SAM & Zero (auto) & 0.167 & \underline{0.083} & 0.298 & \underline{0.000} & 0.290 & \underline{0.000} & 0.080 & \underline{0.011} & 0.037 & 0.354 & 0.224 & 0.207 \\
SCLIP & Zero & 0.103 & 0.000 & 0.117 & \underline{0.000} & 0.231 & \underline{0.000} & 0.116 & 0.002 & 0.026 & 0.426 & 0.112 & 0.161 \\
ProxyCLIP & Zero & 0.127 & 0.000 & 0.123 & \underline{0.000} & 0.230 & \underline{0.000} & 0.098 & 0.003 & 0.029 & 0.417 & 0.025 & 0.150 \\
MedSAM & Zero (box) & 0.021 & 0.000 & 0.161 & \underline{0.000} & 0.224 & \underline{0.000} & 0.112 & 0.000 & 0.019 & 0.381 & 0.214 & 0.162 \\
LISA & Zero & 0.052 & \textbf{0.250} & 0.173 & \underline{0.000} & 0.163 & \underline{0.000} & 0.145 & 0.003 & 0.031 & 0.179 & 0.350 & 0.156 \\
MaskCLIP & Zero & 0.088 & 0.000 & 0.089 & \underline{0.000} & 0.176 & \underline{0.000} & 0.060 & 0.001 & 0.028 & 0.379 & 0.022 & 0.120 \\
Text4Seg & Zero & 0.023 & \underline{0.083} & 0.027 & \textbf{1.000} & 0.068 & \textbf{0.889} & 0.065 & \textbf{0.612} & 0.014 & 0.139 & 0.034 & 0.053 \\
\midrule
\multicolumn{14}{l}{\emph{Interface tuning: backbone frozen, only the segmentation interface is trained ($K=10$)}} \\
\midrule
ProxyCLIP & Interface & \textbf{0.554} & \textbf{1.000} & \underline{0.548} & 0.407 & \underline{0.556} & 0.778 & \underline{0.232} & 0.496 & 0.007 & \textbf{0.831} & \underline{0.440} & \textbf{0.453} \\
MaskCLIP & Interface & \underline{0.435} & 0.000 & 0.472 & 0.111 & 0.523 & 0.519 & \textbf{0.251} & 0.176 & \textbf{0.118} & 0.767 & \textbf{0.457} & \underline{0.432} \\
LISA & Interface & 0.155 & 0.083 & \textbf{0.554} & 0.000 & \textbf{0.601} & 0.000 & 0.159 & 0.279 & 0.000 & 0.759 & 0.440 & 0.381 \\
SCLIP & Interface & 0.072 & \textbf{1.000} & 0.386 & \underline{0.519} & 0.482 & 0.704 & 0.138 & \textbf{0.849} & 0.000 & 0.685 & 0.430 & 0.313 \\
MedPLIB & Interface & 0.296 & 0.000 & 0.331 & 0.148 & 0.318 & 0.000 & 0.128 & 0.038 & \underline{0.098} & \underline{0.813} & 0.262 & 0.321 \\
LENS-LLaVA-OV-7B & Interface (light) & 0.249 & 0.179 & 0.476 & 0.000 & 0.331 & 0.000 & 0.151 & 0.045 & 0.045 & 0.581 & 0.139 & 0.282 \\
F-LMM & Interface (light) & 0.092 & \underline{0.702} & 0.444 & 0.000 & 0.231 & \textbf{0.926} & 0.154 & \underline{0.667} & 0.000 & 0.707 & 0.417 & 0.292 \\
LENS-LLaVA-1.5-7B & Interface (light) & 0.199 & 0.143 & 0.072 & 0.074 & 0.316 & 0.000 & 0.138 & 0.118 & 0.001 & 0.561 & 0.176 & 0.209 \\
GLaMM & Interface & 0.038 & 0.000 & 0.152 & 0.000 & 0.301 & 0.000 & 0.104 & 0.000 & 0.018 & 0.565 & 0.207 & 0.198 \\
LENS-Qwen2VL-2B & Interface (light) & 0.096 & 0.000 & 0.198 & 0.185 & 0.232 & 0.000 & 0.142 & 0.170 & 0.028 & 0.575 & 0.222 & 0.213 \\
STAMP-2B & Interface & 0.075 & 0.000 & 0.351 & 0.000 & 0.309 & 0.000 & 0.192 & 0.000 & 0.056 & 0.605 & 0.294 & 0.269 \\
Text4Seg & Interface & 0.044 & 0.417 & 0.091 & \textbf{0.889} & 0.168 & \underline{0.852} & 0.049 & 0.496 & 0.009 & 0.276 & 0.054 & 0.099 \\
\midrule
\multicolumn{14}{l}{\emph{Backbone tuning: the backbone is adapted together with the interface, via LoRA or full updates ($K=10$)}} \\
\midrule
MedSAM3 & Backbone (LoRA) & \textbf{0.592} & 0.083 & \textbf{0.793} & 0.000 & \textbf{0.847} & 0.000 & \textbf{0.404} & 0.024 & \textbf{0.743} & \textbf{0.898} & \textbf{0.775} & \textbf{0.722} \\
U-Net & Scratch & \underline{0.472} & 0.274 & 0.324 & 0.000 & 0.397 & 0.000 & \underline{0.337} & 0.364 & \underline{0.489} & 0.803 & 0.357 & \underline{0.454} \\
ProxyCLIP & Backbone & 0.296 & \textbf{1.000} & 0.519 & 0.630 & 0.538 & 0.926 & 0.206 & 0.645 & 0.004 & 0.820 & 0.411 & 0.399 \\
U-Net & Scratch (10-shot) & 0.450 & 0.083 & 0.258 & 0.000 & 0.354 & 0.000 & 0.287 & 0.486 & 0.473 & 0.688 & 0.311 & 0.403 \\
LISA & Backbone (LoRA) & 0.155 & 0.131 & 0.556 & 0.000 & \underline{0.604} & 0.000 & 0.200 & 0.225 & 0.000 & 0.762 & 0.461 & 0.391 \\
LISA & Backbone & 0.209 & 0.131 & \underline{0.580} & 0.000 & 0.558 & 0.000 & 0.147 & 0.347 & 0.001 & 0.729 & \underline{0.475} & 0.385 \\
MedPLIB & Backbone & 0.400 & 0.000 & 0.417 & 0.000 & 0.342 & 0.000 & 0.135 & 0.000 & 0.158 & \underline{0.825} & 0.332 & 0.373 \\
MaskCLIP & Backbone & 0.323 & \textbf{1.000} & 0.537 & 0.074 & 0.452 & \underline{0.963} & 0.091 & 0.604 & 0.060 & 0.687 & 0.346 & 0.357 \\
STAMP-7B & Backbone (LoRA) & 0.066 & 0.500 & 0.571 & 0.000 & 0.504 & 0.000 & 0.204 & 0.150 & 0.029 & 0.759 & 0.474 & 0.372 \\
SCLIP & Backbone & 0.096 & \textbf{1.000} & 0.291 & \underline{0.852} & 0.406 & \textbf{1.000} & 0.135 & \textbf{0.738} & 0.013 & 0.783 & 0.358 & 0.297 \\
GLaMM & Backbone & 0.129 & 0.000 & 0.353 & 0.000 & 0.376 & 0.000 & 0.164 & 0.000 & 0.043 & 0.645 & 0.417 & 0.304 \\
SAM & Backbone & 0.265 & 0.131 & 0.264 & 0.111 & 0.382 & 0.037 & 0.109 & 0.310 & 0.003 & 0.477 & 0.036 & 0.219 \\
STAMP-2B & Backbone & 0.063 & 0.000 & 0.229 & 0.000 & 0.324 & 0.000 & 0.153 & 0.000 & 0.038 & 0.638 & 0.275 & 0.246 \\
MedSAM & Backbone (box) & 0.062 & 0.000 & 0.156 & 0.000 & 0.225 & 0.000 & 0.141 & 0.000 & 0.020 & 0.399 & 0.218 & 0.175 \\
Text4Seg & Backbone (LoRA) & 0.056 & 0.464 & 0.053 & \textbf{0.926} & 0.115 & 0.926 & 0.060 & \underline{0.687} & 0.006 & 0.247 & 0.035 & 0.082 \\
Text4Seg & Backbone & 0.048 & \underline{0.833} & 0.185 & 0.333 & -- & -- & -- & -- & -- & -- & -- & 0.117 \\
\bottomrule
\end{tabular}
}
\caption{Performance on \benchmark under the 10-shot IID mode.\textbf{Bold} and \underline{underline} denote the best and second-best, respectively.}
\label{tab:organ_iid}
\end{table*}

